Smoothed Online Convex Optimization in High Dimensions via Online Balanced Descent

We study Smoothed Online Convex Optimization, a version of online convex optimization where the learner incurs a penalty for changing her actions between rounds. Given a $\Omega(\sqrt{d})$ lower bound on the competitive ratio of any online algorithm, where $d$ is the dimension of the action space, we ask under what conditions this bound can be beaten. We introduce a novel algorithmic framework for this problem, Online Balanced Descent (OBD), which works by iteratively projecting the previous point onto a carefully chosen level set of the current cost function so as to balance the switching costs and hitting costs. We demonstrate the generality of the OBD framework by showing how, with different choices of "balance," OBD can improve upon state-of-the-art performance guarantees for both competitive ratio and regret, in particular, OBD is the first algorithm to achieve a dimension-free competitive ratio, $3 + O(1/\alpha)$, for locally polyhedral costs, where $\alpha$ measures the "steepness" of the costs. We also prove bounds on the dynamic regret of OBD when the balance is performed in the dual space that are dimension-free and imply that OBD has sublinear static regret.

==> simulation.tex <==
In this section, we try to test the performance of online projection under various settings. 
\subsection{Quadratic cost}
We set $\beta = 0.5$, and $f_t(x) = \| A_t x - y_t\|_2^2$, where $A_t$ is a random $d \times d$ matrix with fixed condition number (default set to 10), and $y_t \in \mathcal{Y} \subset \mathbb{R}^d$, and the diameter of $\mathcal{Y}$ is fixed (default set to 10). We vary the number of dimension $d$ for the problem, for each dimension, we run 10 trials, the result is shown in Fig. \ref{fig: cr_vs_dim}.  
\begin{figure}[h!]
	\centering
	\includegraphics[width=.5\textwidth]{CR_vs_dimension}
	\caption{Competitive ratio against dimension while keeping the diameter of the feasible set constant}
	\label{fig: cr_vs_dim}
\end{figure}
Fig. \ref{fig: cr_vs_dim} shows that, surprisingly, the competitive ratio of Algorithm \ref{alg: online-projection} decreases as the dimension of the problem increases. 

\subsection{Linear cost}
We set $\beta = 0.5$, and $f_t(x) = \| A_t x - y_t\|_2$, where $A_t$ is a random $d \times d$ matrix with fixed condition number (default set to 10), and $y_t \in \mathcal{Y} \subset \mathbb{R}^d$, and the diameter of $\mathcal{Y}$ is fixed (default set to 10). We vary the number of dimension $d$ for the problem, for each dimension, we run 10 trials, the result is shown in Fig. \ref{fig: cr_vs_dim_lin}.
 \begin{figure}[h!]
	\centering
	\includegraphics[width=.5\textwidth]{CR_vs_dimension_lin}
	\caption{Competitive ratio against dimension while keeping the diameter of the feasible set constant}
	\label{fig: cr_vs_dim_lin}
\end{figure}

==> strongly_convex.tex <==
In this section we discuss performance guarantee for strongly convex cost functions with respect to the norm of switching cost, i.e., for all $t$, there exist $m>0$, such that $f_t(x) - f_t(y) \le \nabla f_t(y)^T (x-y) + \frac{m}{2}\norm{x-y}^2$. 
 \todo{can we do something about this case?}

% For this class of function, we slightly modify Algorithm \ref{alg: online-projection}.
%
% The overall idea is the following:
% \begin{enumerate}
% 	\item We can show that if all $f_t$ are $m$ strongly convex, then $\norm{x_t^* - v_t} \le h(m)$, for some $h$ to be determined later.
% 	\item Hence, instead of projecting to a sublevel set such that the movement cost and hit cost is balanced, we can make potentially bolder move that ensures $\norm{x_t - v_t} \le h(m)$, while still respecting the geometry (that $x_{t-1} - x_t \in \partial f_t(x_t)$). (this step need to be more rigorous, but let's suppose this can be done...)
% 	\item If $H_t \le H_t^*$, then $x_t$ is already in the $h_m$ neighborhood. We can follow the same step.
% 	\item If $H_t > H_t^*$, then we need the analogous result for Lemma \ref{lem: potential-change}. However, we cannot get the result without making further assumption about the cost sequence, we need something like $\norm{v_t - v_{t-1}} \le K$ only happening $O(1)$ times, and appeal to the fact that $ \norm{x_t - v_t} + \norm{v_t - v_{t-1}} + \norm{v_{t-1}-x_{t-1}} \le \norm{x_t - x_{t-1}}$.
% \end{enumerate}
%
% \begin{algorithm}
% 	\begin{algorithmic}[1]
% 			\FOR{$t=1, \ldots, T$}
% 			\STATE If $\norm{x_{t-1}-v_t} \le \beta f_t(v_t)$, then set $x_t = v_t$.
% 			\STATE Otherwise, choose the $m$-sublevel set $K_l$ of $f_t$, i.e., $K_l = \{ x | f_t(x) \le l\}$, such that,
% 			 $d(x_{t-1}, K_l) = \beta l$
% 			\label{projection-step}
% 			 \STATE $x_t = \Pi_{K_l}(x_{t-1})$.
% 			\ENDFOR
% 	\end{algorithmic}
% \caption{Online projection algorithm for $m$-strongly convex functions}
% \label{alg: online-projection-sconvex}
% \end{algorithm}
%
